Interactive Continual Learning Architecture for Long-Term Personalization of Home Service Robots

For robots to perform assistive tasks in unstructured home environments, they must learn and reason on the semantic knowledge of the environments. Despite a resurgence in the development of semantic reasoning architectures, these methods assume that all the training data is available a priori. However, each user's environment is unique and can continue to change over time, which makes these methods unsuitable for personalized home service robots. Although research in continual learning develops methods that can learn and adapt over time, most of these methods are tested in the narrow context of object classification on static image datasets. In this paper, we combine ideas from continual learning, semantic reasoning, and interactive machine learning literature and develop a novel interactive continual learning architecture for continual learning of semantic knowledge in a home environment through human-robot interaction. The architecture builds on core cognitive principles of learning and memory for efficient and real-time learning of new knowledge from humans. We integrate our architecture with a physical mobile manipulator robot and perform extensive system evaluations in a laboratory environment over two months. Our results demonstrate the effectiveness of our architecture to allow a physical robot to continually adapt to the changes in the environment from limited data provided by the users (experimenters), and use the learned knowledge to perform object fetching tasks.

==> limitations.tex <==

altough only object serach tasks for now. Future we will perform learning non-causal tasks like setting up a table for breakfast and causal tasks which could be learned by the person actually showing the sequence of actions and objects used to perform the task. 

==> norm_inferencing.tex <==
\section{Learning Norms}
\label{sec:inferencing}

\noindent 

\begin{algorithm}
\caption{Updating Probabilities Based on Endorsements}
\begin{flushleft}
        \textbf{input:} $p$\Comment{Boolean variable if true the action is permissible and false the action is not permissible}\\
        \textbf{input:} $A$\Comment{ Action that the endorsement applies to }\\
        \textbf{input:} $u$\Comment{ User that gave the endorsement }\\
        \textbf{input:} $O$\Comment{ Object that the endorsement applies to}\\
        \textbf{require:} $X={x_1,x_2,...,x_n}$\Comment{Total objects}\\
        \textbf{require:} $B=\{f_1,...,f_{r}\}$\Comment{The number of endorsements for a particular action by a particular owner} \\
        \textbf{require:} $U=\{u_1,...,u_m\}$\Comment{The number of endorsements for a particular action by all owners} \\
        \textbf{require:} $W_u=$\Comment{The threshold weight of endorsements by 
        a user that must be passed to use their endorsements to infer norms} \\
        \textbf{require:} $W_t$\Comment{The threshold weight of endorsements by 
        all users that must be passed to use their endorsements to infer norms} \\
        \textbf{require:} $E=\{e_A1,...,e_Am\}$\Comment{Endorsement weights for each action made by all users.} \\
\end{flushleft}
\begin{algorithmic}[1]
\State $O(A).lower\_probability=O(A).lower\_probability * O(A).endorsment\_weight + float(p)$\Comment{Update the lower probability that the action can be performed}
\State $O(A).upper\_probability=O(A).upper\_probability * O(A).endorsment\_weight + float(p)$\Comment{Update the higher probability that the action can be performed}
\State $O(A).endorsment\_weight+=1$\Comment{Update the endorsement weight for that action on this object}
\State $O(A).endorsment\_weight+=1$\Comment{Update the endorsement weight for that action on this object}
\State $u(A).endorsment\_weight+=1$\Comment{Update the endorsement weight for that action by this user}
\State $u(A).endorsment\_weight+=1$\Comment{Update the endorsement weight for that action by this user}
\For{$obj\in O.objs$}\Comment{Loop through each object}
    \If{$obj.is\_owned() \& !obj.user_set_permission(A)$}\Comment{If the object is owned and the permissions for this object were not set by the owner}
        \State $norm_weight = 0$\Comment{Used to calculate the current weighting of the norms applied to this object by previous updates}
        \State $num_owners = obj.num_owners()$
        \For{$own\in obj.owners$}\Comment{Loop through each of the object's owners}
            \If{$own(A).endorsment\_weight <= W_u \&\& E(A) > W_t$}Comment{Use the norm weight of endorsements made by all users if the owner has not made enough endorsements for this action}
                \State $norm_weight += E(A)$
            \ElsIf{$own(A).endorsment\_weight > W_u \&\& u==own$}Comment{Use the norm weight of endorsements made by the owner if the owner is the one who made the endorsement}
                \State $norm\_weight += own(A).endorsment\_weight$
            \ElsIf{$own(A).endorsment\_weight > W_u \&\& u!=own$}\Comment{Use the norm weight of endorsements  made by the owner and subtract the number of owners that apply to this endorsement if the owner is not the one who made the endorsement}
                \State $norm\_weight += own(A).endorsment\_weight$
                \State $num\_owners -= 1$
            \Else\Comment{If none of these conditions are true this update does not apply to this user so remove them from the count}
                \State $num\_owners -= 1$\Comment{find dependency with food items}
            \EndIf
        \EndFor
        \If{$num_owners > 1$}\Comment{Use the norm weight of endorsements made by all users if the owner has not made enough endorsements for this action}
            \State $norm\_weight\_coefficent += 5*tanh((norm\_weight/num_owners-10)/6)+6$
            \State $endorsment\_coefficent = (-1/3)*(tanh(O.get_endorsment_weight(A)/3-2))+2/3$
            \State $action\_new\_a\_value = (norm\_weight\_coefficent * obj.get\_a\_value(A) + endorsment\_coefficent * (1 if permitted else 0)) / (norm_weight_coefficent + endorsment_coefficent)$
            \State $action\_new\_b\_value = (norm\_weight\_coefficent * obj.get\_b\_value(A) + endorsment\_coefficent * (1 if permitted else 0)) / (norm_weight_coefficent + endorsment_coefficent)$
            \State $obj.a(A) = action\_new\_a\_value$
            \State $obj.b(A) = action\_new\_b\_value$
        \EndIf
    \EndIf
\EndFor

\end{algorithmic}
\end{algorithm}

\subsection{Updating Permissions and Inferring Norms}
When an action endorsement is given to an object by its owner the permission interval for that action is updated. The system attempts to infer ownership norms by applying that endorsement to other objects that share the same owner. The algorithm for this process is shown in ().

\subsection{Inferring Norms From Ownership}

When the ownership of an object is claimed by a user the system attempts to infer norms based on the new owner. 
